Targum -- A Multilingual New Testament Translation Corpus

Many European languages possess rich biblical translation histories, yet existing corpora - in prioritizing linguistic breadth - often fail to capture this depth. To address this gap, we introduce a multilingual corpus of 651 New Testament translations, of which 334 are unique, spanning five languages with 2.4-5.0x more translations per language than any prior corpus: English (194 unique versions from 390 total), French (41 from 78), Italian (17 from 33), Polish (29 from 48), and Spanish (53 from 102). Aggregated from 12 online biblical libraries and one preexisting corpus, each translation is annotated with metadata that maps the text to a standardized identifier for the work, its specific edition, and its year of revision. This canonicalization allows researchers to define "uniqueness" for their own needs: they can perform micro-level analyses on translation families, such as the KJV lineage, or conduct macro-level studies by deduplicating closely related texts. By providing the first multilingual resource with sufficient depth per language for flexible, multilevel analysis, the corpus fills a gap in the quantitative study of translation history.

==> tables/metadata_fields.tex <==
\begin{tabular}{lll}
    \toprule
    Field & Description & Example \\
    \midrule
    \texttt{site} & Source website & \texttt{laparola.net} \\
    \texttt{iso} & ISO 639-3 language code & \texttt{eng} \\
    \texttt{translation\_id} & Site-specific translation identifier & \texttt{asv} \\
    \texttt{translation\_name} & Full translation name & \texttt{American Standard Version} \\
    \texttt{translation\_abbr} & Common abbreviation & \texttt{ASV} \\
    \texttt{canonical\_id} & Groups all instances of the same translation work & \texttt{king-james-version} \\
    \texttt{canonical\_version} & Edition label; often a year but may encode more (e.g.\ \texttt{1989-anglicised-catholic}) & \texttt{1769} \\
    \texttt{canonical\_year} & Integer revision year; places the edition on the time axis & \texttt{1769} \\
    \texttt{num\_chapters} & Number of NT chapters present & \texttt{260} \\
    \texttt{num\_verses} & Number of NT verses present & \texttt{7957} \\
    \texttt{num\_words} & Total word count & \texttt{179836} \\
    \texttt{copyright\_status} & Copyright classification; accompanied by a reasoning field (not shown) & \texttt{public\_domain} \\
    \bottomrule
\end{tabular}
